DOLOMITES: Domain-Specific Long-Form Methodical Tasks

Experts in various fields routinely perform methodical writing tasks to plan, organize, and report their work. From a clinician writing a differential diagnosis for a patient, to a teacher writing a lesson plan for students, these tasks are pervasive, requiring to methodically generate structured long-form output for a given input. We develop a typology of methodical tasks structured in the form of a task objective, procedure, input, and output, and introduce DoLoMiTes, a novel benchmark with specifications for 519 such tasks elicited from hundreds of experts from across 25 fields. Our benchmark further contains specific instantiations of methodical tasks with concrete input and output examples (1,857 in total) which we obtain by collecting expert revisions of up to 10 model-generated examples of each task. We use these examples to evaluate contemporary language models highlighting that automating methodical tasks is a challenging long-form generation problem, as it requires performing complex inferences, while drawing upon the given context as well as domain knowledge.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/conclusion.tex <==
\section{Conclusion}

% \todo[inline]{TODO: Add conclusion text.}

Language models hold great promise to be used as writing assistants for assisting domain experts from various fields. Through \textsc{Dolomites}, we propose a benchmark that is closely tied to realistic use cases of domain experts for which they might like to use language models. The generalization of these use cases as methodical tasks provides a way to study capabilities of language models across tasks and domains. Since these tasks are pervasive across fields, we believe that models that are capable of assisting with these tasks have the potential to impact a range of fields. We verify that our tasks are representative tasks from the corresponding field and highlight the societal implications of using language models to propose initial outputs for the tasks. Evaluation of contemporary language models suggests that there is a large room for models to improve on generating outputs for our tasks.

==> sections/dataset.tex <==
\section{\textsc{Dolomites}: Data Curation}
\label{sec:data}

\input{tables/tasks_mirella}

\subsection{Task Collection} 
\label{sec:task_collection}

In our data curation process, we first collect a typology of realistic tasks that span multiple fields. These tasks are not meant to be comprehensive, but instead just represent a reasonable subset of realistic use cases from various fields.
% This is aimed to understand how language models could be of assistance to domain experts.

\subsubsection{Setup}

\paragraph{Participants.} We recruit 266 participants for our study from Prolific. Participants are qualified as experts if they have formal education in the field, and at least 3 years of work experience in the field. Additional details about the participants' backgrounds are provided in Appendix~\ref{app:annotation}. We recruit experts from 25 different fields, shown in Table~\ref{tab:tasks_all}, aiming for a broad coverage of various disciplines.

\paragraph{Annotation Task.} We ask each annotator to provide descriptions of two tasks that they perform in their professional life where an AI model can assist. We provide the criteria listed in section~\ref{subsec:methodical_tasks} to the annotators. For each task, annotators are asked to fill in predefined fields (task objective, procedure, input and output sections, additional notes), the same way as the tasks shown in Figure~\ref{fig:sample_tasks}.
% A predefined template allows us to scale to many tasks and domains while keeping a standard instruction format \citep{khashabi2020unifiedqa,mishra2021cross,wang-etal-2022-super}. 
We ask annotators to give a thorough description of the task, as if they are teaching a beginner in the field how to perform this task. Finally, we also ask them to provide us a list of URLs to web documents that contain examples of this task. Instructions and interface screenshots are in Appendix~\ref{app:annotation}.

% We also emphasize that these tasks should involve writing a structured document which has well-defined sections.

% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=2\columnwidth]{images/dolomites_field_distrib.pdf}
%     \caption{Distribution of fields in the \textsc{Dolomites} task collection.}
%     \vspace{-10pt}
%     \label{fig:field_distrib}
% \end{figure*}

\subsubsection{Task Analysis}

After collecting the initial set of tasks, we filter them manually to ensure that they meet the criteria outlined in section~\ref{sec:problem}. This results in a total of 519 tasks. We find that there are very few tasks from a field that are highly similar. Tasks which are somewhat similar still vary based on precisely what is expected in the input and output sections.

% Distribution across fields
Table~\ref{tab:tasks_all} provides the number of tasks across fields and the task objective of a sample task from each field. Most fields have at least 20 tasks, with some exceptions, where we were not able to recruit as many experts. As tasks in \textsc{Dolomites} come from a diverse set of fields, AI models that can assist with these tasks can potentially serve the needs of experts across fields.

Collectively, tasks in \textsc{Dolomites} are cognitively demanding and versatile in the types of reasoning they require. For instance, a diagnostic task in medicine requires inductive reasoning to go from particular symptoms to a general diagnosis. Whereas, in legal analysis, deductive reasoning is required to reason about how laws are interpreted in a specific case and analogical reasoning is needed as lawyers compare current cases with precedents. Similarly, in software application design, abstract reasoning is important for creating modular application designs while creativity is necessary for certain tasks in the visual arts. While it is hard to characterize each task with the type of reasoning required, each methodical task can be boiled down to \textbf{analysis} of the input, drawing an \textbf{inference} based on the input and domain-specific knowledge and finally, a \textbf{justification} provided in writing.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=2\columnwidth,keepaspectratio]{images/task_validation.pdf}
    \caption{Validation of tasks in the \textsc{Dolomites} task collection.}
    \vspace{-10pt}
    \label{fig:task_validation}
\end{figure*}

\subsection{Task Validation}
\label{sec:task_validation}

We validate our collection of tasks by consulting an independent group of experts. Each task is evaluated by three independent experts from the field to which the task belongs. Specifically, we collect Likert ratings for each task on the following axes (the precise description for each item on the scale is provided in Appendix \ref{app:annotation}):

\begin{itemize}
\itemsep0em 
\item \textbf{Representativeness}: How likely is this task to be conducted by an expert in your field?
\item \textbf{Complexity}: How would you rate the complexity of this task?
\item \textbf{Time Required}: How much time is typically required to complete this task?
\item \textbf{Usefulness}: Would you or other experts find it useful if an AI system could be used to propose initial outputs for this task (which may be lacking), that can be validated and improved by experts?
\end{itemize}

\paragraph{Societal Implications.} Prior work has shown that using language model as writing assistants has the capability to significantly benefit productivity of experts \citep{eloundou2023gpts,noy2023experimental,dell2023navigating}. Beyond improving productivity, we were interested in expert opinions about the societal implications of using language models as writing assistants. Hence, for each task, we also ask the following questions to evaluate societal implications, where each question requires a free-text response in addition to a Likert rating.
\begin{itemize}
\itemsep0em 
\item \textbf{Anonymity Required}: Is it important to ensure anonymity of any individuals or organizations mentioned if an AI system is used for conducting this task? This may be the case if there is sensitive information in the input that should not be stored or accidentally leaked by an AI system.
\item \textbf{Biased Outcomes}: Could relying on automatically generated outputs for this task result in biased or potentially harmful decisions for certain groups of people?
\item \textbf{Ethical Considerations}: Are there ethical considerations associated with the use of AI systems for this task? This can include privacy issues, moral issues, copyright issues or any other issues.
\item \textbf{Workforce Impact}: Could partial automation of this task potentially have an impact on the workforce in the short term?
\item \textbf{Accessibility Requirements}: Does the use of AI systems for this task require making exceptional considerations for ensuring accessibility to all users? For instance, a task that requires producing visual data might pose challenges for people with visual or motor disabilities.
\end{itemize}

\subsubsection{Results}

The main statistics based on task validation are presented in Figure~\ref{fig:task_validation}. We find the tasks in the \textsc{Dolomites} task collection are likely ($\sim$76\%) to be conducted by some experts in the field, reflecting the practical nature of these tasks. Further, a majority of tasks are medium or high complexity, meaning that they require a moderate amount of field expertise (few years of experience) or immense field expertise (several years of experience) respectively. While they are complex tasks, the judgements about the time taken for these tasks reveals that most of them ($\sim$ 61\%) would take an expert from 1 hour to 7 days. We think the level of difficulty is appropriate as, although the tasks are challenging, the time judgements suggest that it is conceivable that language models could be useful assistants for these tasks. Finally, an overwhelming majority of experts would be interested ($\sim$62\%) or open to trying ($\sim$32\%) to use a language model that proposes initial outputs for the task.

\subsubsection{Results: Societal Implications}

\begin{itemize}[leftmargin=*]
    \item \textbf{Anonymity Required}: The need for anonymity emerged as a concern for a significant number of tasks ($\sim$58\%) across fields. In fields like medicine, psychology, and law, experts emphasized the importance of protecting patient/client confidentiality (\textit{ "Patient confidentiality is imperative, so no information should be stored by the system once the report has been created.", "CBT formulations are incredibly personal... Anonymity is crucial to protect the privacy of individuals and organizations", "Client confidentiality is essential. I would not trust an AI with any information that can be linked back to the client"}). Similarly, it was emphasized that proprietary information and trade secrets should be kept private in other fields like business. Further research on better privacy protection practices with language model use is essential for enabling experts to use these models \citep{brown2022does}.
    \item \textbf{Biased Outcomes}: Experts believe that using language model responses for these tasks without careful perusal can result in biased outcomes ($\sim$56\% of tasks). Concerns about data bias, due to unrepresentative training data, and algorithmic bias, through optimization, were brought up. In many such cases, experts emphasized that AI systems may learn and perpetuate existing societal biases, which could affect marginalized or underrepresented groups (\textit{"AI systems are only as good as the data they are fed, and a lot of data we have collected have biases because they were originally collected or analysed by humans."}, \textit{"AI has been known to show bias against certain groups of people... This could lead to unethical decisions and bias opinions especially for minority groups."}). We echo these sentiments and emphasize that experts must carefully vet the responses these systems before using them for their work.

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=2\columnwidth]{images/example_creation.pdf}
    \caption{Method for constructing examples of tasks in \textsc{Dolomites}.}
    \vspace{-5pt}
    \label{fig:example_creation}
\end{figure*}

    \item \textbf{Ethical Implications}: Topics such as copyright issues, privacy issues and stifling of human creativity due to overreliance on AI were brought up. (\textit{"There are ethical considerations associated with the use of AI systems for this task, particularly regarding privacy and confidentiality... Additionally, transparency about the use of AI systems and informed consent from individuals whose data is processed are essential ethical considerations."}, \textit{"Privacy issues! Concerns with accuracy on education and nuance. HUGE issues if goals of care... are mistakenly input or have the wrong nuance."}, \textit{"The ethical side comes after this I should think, when humans make decisions based on the content provided... It doesn't have the sensitivity or is aware of the political climate and relationships that are present."}). These are complex challenges, which required tailored approaches depending on the ethical concern and task. Since language models are now widely accessible, we believe that considerations associated with their use as writing assistants should be preemptively discussed by stakeholders.
    \item \textbf{Workforce Impact}: Many experts ($\sim$43\%) recognized that partial automation of writing tasks through AI systems is likely to impact the workforce in the short term, potentially leading to changes in job roles or skill requirements. At the same time, experts were positive that this would improve productivity and change the nature of work (\textit{"While automation might streamline certain aspects, it could also lead to shifts in job roles or requirements for new skills."}, \textit{"AI is already having a big impact in the field of visual arts, as any other group within the arts, photography will likely be affected by this."}, \textit{"This is the type of task in a larger firm a paralegal or someone else assisting an attorney could undertake. Having an AI tool would streamline the process greatly and would free up staff to handle more complicated tasks. This could potentially lead to less jobs but it would likely be overall positive."}).
    \item \textbf{Accessibility Requirements}: It is important to ensure that users of all backgrounds and capabilities have equal access to language models. A significant number of tasks ($\sim40\%$) were rated as requiring exceptional considerations to be made for ensuring accessibility to all users. The comments provide insights about how such considerations can be made, so that users with differing capabilities are not disadvantaged. (\textit{"It is important that the lesson plan is accessible for all. This includes those with disabilities."}, \textit{"Accessibility needs to be taken into account in the development of the model... This could include literacy/numeracy levels as well as any other identified disabilties or needs."}, \textit{"AI systems should adapt their output to accommodate for special needs (such as producing audio output for those who have visual disabilities). For reasons of fairness and equality, AI systems should account for the experiences of all users."}).
\end{itemize}

Experts across fields highlighted that while language models can improve productivity when used as writing assistants, human oversight is important for responsible use of these technologies. 

\subsection{Example Collection}
\label{sec:example_collection}

To evaluate models for their capabilities to assist experts with their tasks, we create examples of the tasks in our collection. These are samples of the input and output sections of each task with concrete details. Examples are created in a human-in-the-loop fashion, where initial examples of a task are generated by a model, which are then post-edited by the same expert who provided the task. We describe this process below.

\subsubsection{Retrieval-Augmented Generation}

We believe that samples of the tasks are partially available in documents on the web. Hence, we retrieve relevant web documents for each task and generate examples by prompting models with passages from these documents as context. This process is depicted in Figure~\ref{fig:example_creation}.

\begin{enumerate}
    \item \textbf{Query Formulation}: Given the task description, we first need to find more specific queries that could potentially result in relevant web documents. For example, for a task that involves writing a catalog entry for an art exhibition, search queries with more specific entities (such as \textit{"renaissance art exhibition catalog entry"}, \textit{"picasso guernica catalog entry"}, \textit{"The Great Wave off Kanagawa catalog entry"}) are likely to result in documents that contain examples of the task. To generate search queries for a task, we prompt Bard \citep{manyika2023overview} (with 1 exemplar) with the task objective and instruct it to generate more specific queries that can help find web documents which contain demonstrations of the task (Table~\ref{tab:query_formulation_prompt}). We generate 10 search queries for each task. Additionally, we restrict search to reliable and authoritative sources. These are collected by prompting Bard (with 1 exemplar) with the task objective for URLs to domain names which will be useful to find real examples for the given task (Table~\ref{tab:domain_name_prompt} in Appendix~\ref{app:annotation}).
    \item \textbf{Evidence Collection}: Using each search query, we gather the top-10 documents after performing a Google search, while restricting to relevant domains (with the \texttt{site:} operator in the query). Documents are split into passages of 4000 characters with a 100 character sliding window.
    \item \textbf{Conditional Generation}: Having gathered evidence which may contain demonstrations of the task, we generate examples by prompting models with this evidence. We explore a multi-document setting, where passages are sampled from multiple documents and a single document setting, where passages are sampled from a single document. We found that the appropriate choice can depend on the task.\footnote{For instance, a task that requires drafting a legal opinion might benefit from multiple relevant documents whereas a single document might be sufficient for writing the catalog entry for an artwork.} Passages are reranked using an in-house reranker and the top-5 passages are provided as context, along with the task description, to a large language model (Gemini-Ultra \citep{team2023gemini} or Bard in our case), which is asked to generate an example of the task (Table~\ref{tab:example_generation_prompt}). Not all the information mentioned in the task description is required to be present in the context and the language model is allowed to infill content to construct an example. We generate up to 10 examples for each task.
\end{enumerate}

\subsubsection{Expert Post-Editing}

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\textwidth]{images/editing_qa_only.pdf}
    \caption{Expert judgements of the original examples according to three criteria - adherence to task structure, level of detail and factual correctness.}
    % \vspace{-5pt}
    \label{fig:editing_qa}
\end{figure*}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\columnwidth,keepaspectratio]{images/edit_distance_dist.pdf}
    \caption{Histogram of the word-level edit distances between the original and post-edited example.}
    \vspace{-10pt}
    \label{fig:edit_dists}
\end{figure}

Model-generated examples, even though they are based on retrieved web documents, could have many issues. Firstly, the example may not adhere to structure specified in the task description. Secondly, there might be factual inconsistencies or inaccuracies in the generated example. Finally, examples may be lacking in depth, or be vague in providing details, such that they do not resemble what an expert might write.

To fix these issues in the examples, we present the examples to the expert who wrote the task for post-editing. They are asked to choose the most plausible example of four choices of examples, that are generated either using Gemini-Ultra or Bard, and use single or multi-document evidences. For the chosen example, we first ask them to label the example for three criteria on a Likert scale: adherence to task structure, factual correctness, and level of detail. They are also shown 1) the evidence passages for the example and 2) a generated critique (generated using Gemini-Ultra with the prompt in Table~\ref{tab:critique_prompt}) of the example, that may not be comprehensive, to aid them in identifying issues with the example. The critique is provided to make post-editing more efficient. They are required to fix any valid issues they recognize in the example as well as any valid issues identified by the critique.

\input{tables/edit_stats}

\subsection{Example Quality Analysis}

\subsubsection{Automatic Analysis}

Expert judgements of their chosen examples are shown in Figures~\ref{fig:editing_qa}. We find that a majority of the examples already follow the task structure ($\sim$85\%) according to experts and most of the examples are \textit{probably} or \textit{definitely} correct. However, a large majority of examples are lacking in depth. This means that most experts find that while the generated examples follow the basic structure of the task, they could be more detailed.

We show a histogram of the word-level edit distance between the original and edited example in Figure~\ref{fig:edit_dists} and relevant statistics of the original and post-edited examples in Table~\ref{tab:edit_stats}. The histogram suggests that on average, there are significant changes made to the original examples during post-editing. Since most experts judge that examples are lacking in depth, the edited examples are expectedly much longer on average. The edited examples also adhere better to the task description (on average, 97.67\% sections in the task description are found in the edited examples compared to 92.81\% in the original examples). Finally, we compute readability scores of the examples as a noisy approximation of the complexity and level of detail in the text. Specifically, we compute the Flesch-Kincaid Grade Level \citep{kincaid1975derivation}. Higher readability values indicate that a piece of text requires more formal education and expertise to understand. We find that post-edited examples have higher scores, possibly indicating higher level of technical depth.

\subsubsection{Risk of Memorization}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth,height=5cm]{images/ngram_overlaps_nltk_cosine.pdf}
    \caption{Histogram of Cosine similarities computed based on the n-grams in the post-edited examples and evidences used as context.}
    \vspace{-5pt}
    \label{fig:overlap}
\end{figure}

Examples in \textsc{Dolomites} are created by conditioning on passages from web documents that may contain demonstrations of the tasks. We do not require these documents to contain complete examples of the task, and models are allowed to infill information to create an example. However, if these documents are seen and memorized by models during large-scale pretraining on the web, it might be difficult to conduct a clean evaluation. We evaluate the extent of this issue by computing the similarity of the post-edited examples to the evidence passages provided during generation. Specifically, we show a histogram of the Cosine similarities between the n-grams found in the post-edited examples and evidences used as context in Figure~\ref{fig:overlap}. We find that the similarities to retrieved passages are fairly low in most examples, which suggests a low risk of memorization due to pretraining.

% \subsubsection{Risk of Model Bias}

% \todo[inline]{TODO: Add discussion of model bias.}


==> sections/ethical.tex <==
\section{Ethical Considerations}

The motivation of our work is not to advocate for AI systems to replace experts with their writing tasks. Instead, we consider a scenario where AI systems can act as tools for experts to amplify their problem-solving capabilities \citep{engelbart2023augmenting} and perform their tasks more efficiently so they can focus on more complex problem-solving acitivities. We recognize that human interaction is irreplaceable for many aspects of our jobs, including building relationships and empathy with other people.

==> sections/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\input{tables/results_std_and_nli_test}

\paragraph{Setup.} We create a dev-test split for \textsc{Dolomites}, where we include 820 examples in the dev set and 1037 examples in the test set. There are 172 seen tasks for which examples are present in both dev and test and 99 unseen tasks for which examples are only present in the test set.
To evaluate models, we prompt models with the task description, the input sections corresponding to an example, and instruct it to generate the output sections for the example. This is done in a zero-shot manner. Hyperparameters and prompts are provided in Appendix~\ref{app:experiments}.

\paragraph{Models.} We consider the following models for evaluation: Claude-3 Haiku and Claude-3 Opus \citep{TheC3},  Command-R-Plus \citep{gomez2024cmdrplus}, Gemini-1.5-Pro \citep{reid2024gemini} and Gemini-Pro \citep{team2023gemini}, GPT-3.5-Turbo and GPT-4 \citep{OpenAI2023GPT4TR}, Mixtral-8x7B-Instruct \citep{jiang2024mixtral} and Mistral-Large \citep{mistral-large}, and OLMo-7B-Instruct \citep{groeneveld2024olmo}. In our selection of models, we aimed to select performant models from various organizations. Further, we tried to include open-source models and models of varying sizes. In all cases, we favored instruction-tuned variants of models because of their better performance on other benchmarks.

\subsection{Evaluation}

\subsubsection{Automatic Metrics}

\paragraph{Conventional Metrics.} Prior work has recognized that that conventional metrics for text generation are lacking in various ways \cite{liu-etal-2016-evaluate,novikova-etal-2017-need,krishna-etal-2021-hurdles}. Nevertheless, for completeness, we consider the following automatic metrics for evaluation: BLEU-4 \cite{papineni-etal-2002-bleu}, ROUGE-L \cite{lin-2004-rouge}, F1-token-overlap, and BLEURT \cite{sellam-etal-2020-bleurt}. In addition, we report the average length of outputs and the average section presence (i.e., the percentage of output sections specified in the task that are present in the generated output, averaged across all examples) as a measure of instruction-following capabilities. Note that the average length of reference outputs is 341.42 tokens.

\paragraph{Round-Trip Factual Consistency.} In this evaluation, we measure the extent to which statements in the reference output are consistent with the statements in the candidate model's output. We conduct this evaluation by computing entailment scores in two setups: 1) forward: considering a reference output section as premise and the corresponding candidate output section as hypothesis and 2) reverse: considering a candidate output section as premise and the corresponding reference output section as hypothesis. Scores are aggregated over all sections and examples. We believe these loosely capture the notions of precision and recall. Finally, we also report the harmonic mean of these two scores. We use the TRUE model \cite{honovich-etal-2022-true-evaluating} to predict entailment scores (ranging from 0 to 1) and report 95\% confidence intervals.


\input{tables/results_autoraters}

\paragraph{LM-based Evaluation.} Language models are being increasingly used as evaluators in recent work \citep{chiang-lee-2023-large}. However, model-generated evaluations can be misleading and biased in unexpected ways \citep{shen-etal-2023-large,wang2023large}.
% Similarly, human judgements are prone to similar undesirable biases \citep{hosking2024human}.
In this evaluation, we use multiple language models as judges to give preferences for a pair of model outputs. While this does not completely alleviate the problem of biased LM judgements, we believe that this is a slightly more reliable evaluation since we are not biased by a single model's biased judgements.

In all comparisons, we use the strongest model, GPT-4, as the base comparison model. We sample 100 pairs of outputs from a candidate model and GPT-4 and ask the evaluator model to judge which output is better quality and provide a justification for its choice. We consider three models as evaluators: GPT-4, Claude-3 Opus and Gemini-Ultra. The win rate is computed by summing up the number of wins for a candidate model plus half the number of ties.

% \subsubsection{Manual Evaluation}

==> sections/intro.tex <==
\section{Introduction}


\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{images/figure1_v2.pdf}
    \caption{\textsc{Dolomites} contains descriptions of 519 methodical tasks elicited from domain experts across various fields. We instantiate these tasks with examples that contain plausible inputs and outputs, formulating a challenging long-form generation problem that requires domain expertise and structured problem-solving.}
    \vspace{-10pt}
    \label{fig:overview}
\end{figure}

% What is the problem?

Experts in various fields regularly use writing as a means for planning and organizing their own work, and as a means of sharing their work with others. For instance, a teacher might draft a lesson plan to plan what they would like to teach in their next class, and a lawyer might draft a patent application for an invention. Experts generally follow a consistent and methodical approach to conduct these writing tasks. In the lesson plan example, a teacher would know the lesson objectives, format and the profile of the class, and they would produce a thorough lesson plan with the topics to be covered and activities to improve learning. Importantly, the teacher follows a systematic procedure to write this lesson plan, using their expertise and what they know about the current context (e.g., the class profile).
% Note that this procedure may exist as a tacit strategy that the teacher has internalized through experience, and not be explicitly written down.

% Why is it interesting and important?

Such \textit{methodical} writing tasks are pervasive across fields. From law to visual arts to engineering, experts across fields conduct tasks that follow a similar systematic design (see a few examples in Figure~\ref{fig:sample_tasks}). The unique feature of these \textit{methodical tasks} is that they loosely follow a standard template for what is usually given as input and what is required from the output. Performing these tasks involves following a structured and consistent procedure as these tasks are conducted by experts on a regular basis. At the same time, these writing tasks tend to be fairly time-consuming, taking from a few hours to several days.

As large language models become more capable and widely accessible to a more sophisticated set of users, they hold great potential for assisting experts with methodical writing tasks. Experts in various fields are already incorporating language models as tools for their work \citep{owens2023nature,mollick2023using} and in the future, they present opportunities for addressing novel use cases in various fields \citep{lee2023benefits,birhane2023,mollick2023using,frankenreiter2022natural,demszky2023using,wang2023scientific,bommasani2021opportunities}. Assistance from models as writing assistants holds potential for increasing efficiency on these procedural tasks, allowing experts to focus on complex problem-solving activities \citep{noy2023experimental}.

% This includes tasks such as performing differential diagnosis, conducting legal research, fact-checking news articles, to name just a few use cases. 

% Why is it hard? (E.g., why do naive approaches fail?)

Given their potential for assisting experts, it would be beneficial to evaluate language models on a realistic set of methodical writing tasks. However, we currently don't have benchmarks that contain a typology of such tasks.
% , i.e., scenarios where they are actively being used as well as scenarios where capable models could improve productivity of experts in the future. 
The most natural source for such data would be query logs \citep{nguyen2016ms,kwiatkowski-etal-2019-natural} or chat histories \citep{zhao2023inthe}. However, these data sources do not specifically reflect domain-specific use cases and do not allow us to study specific use cases in a controlled manner. Compiling such data is therefore challenging as it is not readily available.

% Why hasn't it been solved before? (Or, what's wrong with previous proposed solutions? How does mine differ?)


% In this work, we elicit descriptions of these tasks . 

% These can be generalized as writing tasks that require domain expertise and are conducted in a methodical fashion. Every such \textit{methodical task} contains a standard template for what is usually given as input and what is required from the output. Performing these tasks involves following a structured, consistent procedure as these tasks are conducted by experts on a somewhat regular basis. 
% Importantly, such tasks are pervasive across fields (see a few examples of such tasks in Figure~\ref{fig:sample_tasks}) and understanding how LMs can assist with these tasks can inform us about their usefulness as tools for experts. 

% What are the key components of my approach and results? Also include any specific limitations.

In this work, we bridge this gap by eliciting 519 task descriptions of these methodical writing tasks from 266 experts across 25 different fields (\S\ref{sec:task_collection}) (see a few examples in Figure~\ref{fig:sample_tasks}). These are formatted in a standard way, with a task procedure, input and output. Further analysis of these tasks with an independent group of experts reveals that these are plausible tasks ($\sim$76\% of them are rated as likely conducted by an expert in the field on a regular basis) from their corresponding fields and most experts ($\sim$63\%) would find it useful if they could use a capable AI model as a tool for the task (\S\ref{sec:task_validation}). Our tasks serve as the first collection of realistic use cases of experts spanning multiple domains.

To evaluate the ability of models to assist experts with these tasks, we collect \textit{examples} of the tasks, where we instantiate each task with plausible inputs and outputs (\S\ref{sec:example_collection}). Examples are created semi-automatically, where we first retrieve web documents that could potentially serve as samples of the task, and then generate an example using a language model based on the retrieved web documents. These examples are then significantly post-edited by the same experts (who contributed the task) for improving their adherence to the task description, factual correctness, and level of detail.

We use our benchmark, called \textsc{Dolomites} (Domain-Specific Long-Form Methodical Tasks), to evaluate current models in their ability to generate accurate and detailed outputs (\S\ref{sec:experiments}). We formulate the modeling problem as long-form generation, where models are provided the task description and the example input and asked to generate the example output. Evaluation of generated outputs is challenging, as conventional automatic metrics have shortcomings \citep{schluter-2017-limits,krishna-etal-2021-hurdles} and because these examples require domain-specific knowledge. In addition to conventional metrics, we conduct evaluation through round-trip factual consistency and by using language models as evaluators.

Our results suggest that there is significant headroom in improving performance on these tasks (\S\ref{sec:results}). We hope that \textsc{Dolomites} can serve as a reference for common domain-specific use cases of LMs and as a means for evaluating future models. We release our dataset and code at \url{https://dolomites-benchmark.github.io/}.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=2\columnwidth]{images/dolomites_tasks_sample_v2.pdf}
    \caption{A sample of tasks from law, biology and medicine in \textsc{Dolomites}.}
    \vspace{-5pt}
    \label{fig:sample_tasks}
\end{figure*}


==> sections/intro_old.tex <==
\section{Introduction}

% What is the problem?

Evaluation through standard benchmarks has been a longstanding practice in natural language processing that has enabled us to quantify the performance of NLP systems and broadly, measure progress of the field. Yet, there are few benchmarks that model scenarios which are realistic and encountered by a diverse set of users. More precisely, existing benchmarks lack \textit{ecological validity} \citep{Brunswik1956, Orne1962OnTS}, where trends observed on a given benchmark may not translate to benefits observed in practical applications \citep{bowman2021will}. For benchmarks to be practically useful, it is important that they closely represent real use cases encountered by users \citep{rolnick2024application}.

% Why is it interesting and important?

The landscape of such use cases is constantly in flux, especially as large language models become more capable and widely accessible to a more sophisticated set of users. Notably, experts in various fields are \textit{actively} incorporating language models as tools for their work \citep{owens2023nature,mollick2023using}. This includes tasks such as performing differential diagnosis, conducting legal research, fact-checking news articles, to name just a few use cases. Further improvements in models present opportunities for addressing completely novel use cases in specialized domains \citep{lee2023benefits,birhane2023,mollick2023using,frankenreiter2022natural,demszky2023using,wang2023scientific,bommasani2021opportunities}. However, we don't currently have a good understanding of such use cases, i.e., scenarios where they are actively being used as well as scenarios where capable models could improve productivity of experts in the future.

% Why hasn't it been solved before? (Or, what's wrong with previous proposed solutions? How does mine differ?)
While existing benchmarks \citep{hendryckstest2021,srivastava2022beyond,liang2022holistic} have been greatly beneficial for benchmarking general language comprehension skills, they may not model realistic use-cases. To make evaluation easier, these benchmarks limit their scope to trivia-style question answering problems (sometimes with multiple answer choices). Further, these benchmarks typically test systems for their capabilities in addressing a targeted information need as opposed to open-ended long-form generation. Hence, it may be difficult to form broad conclusions about models based on trends on these benchmarks, especially as performance on them saturates.

% Why is it hard? (E.g., why do naive approaches fail?)

The most natural data for capturing such data would come from user query logs such as those in MSMarco \citep{nguyen2016ms} and Natural Questions \citep{kwiatkowski-etal-2019-natural} or chat histories like ShareGPT or WildChat \citep{zhao2023inthe}. However, these data sources do not cater to domain-specific use cases and do not allow us to study specific use cases in a controlled manner. Compiling such data is therefore challenging as it is not readily available and working with experts to understand their use cases is time-consuming and expensive.

%% Define methodical tasks
% Why are these interesting tasks to study

In this work, we study a specific form of these realistic use cases, i.e., \textbf{domain-specific long-form methodical tasks}, by bringing experts in the loop. These can be generalized as writing tasks that require domain expertise and are conducted in a methodical fashion. Every such \textit{methodical task} contains a standard template for what is usually given as input and what is required from the output. Performing these tasks involves following a structured, consistent procedure as these tasks are conducted by experts on a somewhat regular basis. Importantly, such tasks are pervasive across fields (see a few examples of such tasks in Figure~\ref{fig:sample_tasks}) and understanding how LMs can assist with these tasks can inform us about their usefulness as tools for experts. Assistance from LMs could increase efficiency on these procedural tasks, allowing experts to focus on complex problem-solving activities \citep{noy2023experimental}.

% What are the key components of my approach and results? Also include any specific limitations.

In this work, we elicit 519 task descriptions of these methodical tasks from 266 experts across 25 different fields. These enable us to characterize domain-specific use cases where language models could be useful. Further analysis of these tasks with an independent group of experts reveals that these are plausible tasks ($\sim$76\% of them are rated as likely conducted by an expert in the field on a regular basis) from their corresponding fields and most experts ($\sim$63\%) would find it useful if they could use a capable AI model as a tool for the task. Our tasks serve as the first collection of realistic use cases spanning multiple domains.

In order to evaluate the ability of models to assist experts with these tasks, we collect examples of the tasks, where we instantiate each task with concrete inputs and outputs. The creation of examples is conducted semi-automatically, where we first retrieve web documents that could potentially serve as samples of the task, and then generate an example using a language model based on the retrieved web documents. These examples are then post-edited by the same experts (who contributed the task) for improving their adherence to the task description, factual correctness, and level of detail.

We use our benchmark, called \textsc{Dolomites} (Domain-Specific Long-Form Methodical Tasks), to evaluate contemporary models, as a measure of their helpfulness in assisting experts with conducting the tasks. We formulate the modeling problem for candidate models as long-form generation, where models are provided the task description as well as the example input and asked to generate the example output. Evaluation of generated outputs is challenging, due to commonly discussed shortcomings of automatic metrics for long-form text evaluation \citep{schluter-2017-limits,krishna-etal-2021-hurdles} and because these examples contain domain-specific knowledge. In addition to conventional metrics, we conduct evaluation through round-trip factual consistency and by using language models as evaluators.

Our results suggest that there is significant headroom ... \todo[inline]{TODO: Add discussion of results}

We release our dataset and code at \url{https://dolomites-benchmark.github.io/}.

==> sections/limitations.tex <==
\section{Limitations}

\paragraph{Task Coverage.} The tasks in our collection are not comprehensive and only a sample of tasks from each field are considered. In future work, we hope to further expand the set of tasks to cover a range of scenarios. This might involve a large-scale research effort involving domain experts and NLP researchers. 

\paragraph{Subjectivity in outputs.} Our data contains a single reference output for an example input and does not model the potentially diverse perspectives of various experts from a field. This subjectivity makes model evaluation particularly challenging, because there may not in fact be just one ground truth response \citep{ganguli2023challenges}. While factual consistency metrics do not account for this subjectivity, it is unclear if language model evaluations innately capture this subjectivity in their judgements. More research is needed to ensure language model responses are not penalized for alternative, but valid responses.

\paragraph{Language Coverage.} Tasks and examples in \textsc{Dolomites} are primarily in English. This limits the usefulness of the benchmark when evaluating models as writing assistants for non-English tasks. Future work can consider extending this benchmark to many languages.

\paragraph{Naturalness of data.} In our annotation pipeline, we attempt to simulate a scenario where experts are conducting the task as they typically would in their professional lives. However, there are two potential biases that could affect the naturalness of the examples: 1) the examples are based on web documents (and biased by documents that are publicly available on the internet), and 2) the annotators may be biased in unforeseeable ways and they may not approach the annotation task as they would conduct the task in their work.

\paragraph{Task Scope.} The scope of writing tasks included in \textsc{Dolomites} is limited. We do not consider tasks that involve modalities other than text in input or output, and do not consider the use of sophisticated tools beyond searching. We also do not consider multi-turn settings, where models continually improve their outputs through feedback and revision.


==> sections/problem.tex <==
\section{Problem Formulation}
\label{sec:problem}

\subsection{Methodical Tasks}
\label{subsec:methodical_tasks}

In this section, we first describe the types of writing tasks considered in this work. We refer to these tasks as methodical writing tasks due to two properties that are common to the execution of these tasks. First, each task requires \textbf{structured problem-solving}, where the task follows a specific order where each step logically flows from the previous ones. In the \textit{Medicine} task in Figure~\ref{fig:sample_tasks}, the task first requires producing an assessment of the patient, then listing a plan of care and finally a full evaluation of the patient. Second, every task usually follows a \textbf{consistent execution} across inputs, where there is a standard specification of the input, the output and the procedure for the task. In the \textit{Medicine} task, an expert would typically always be given the patient's subjective and objective data, and would need to produce an assessment, plan of care and full evaluation. Crucially, this task structure and the procedure would mostly stay consistent across patients.
% From writing the plan of care for a patient to writing the design for a software application or conducting a legal analysis on a given matter, methodical tasks share these core properties.

To elicit descriptions of tasks from experts, we operationalize our definition of a methodical task into a standard template. Samples of tasks in this template are in Figure~\ref{fig:sample_tasks}. We require that every task contains a brief \textit{task objective}, a \textit{task procedure} walking a beginner through how this task is conducted, \textit{input and output sections}, which include information that is typically given, and information that needs to be generated for the task given the input sections. Both input and output sections are formatted in the form of section titles and section descriptions. Finally, we collect \textit{additional notes} about the task, which can include best practices or common mistakes, and missing context that is important when conducting the task. This template is aimed to capture a self-contained description of the process of conducting each task.

% Consider the examples from Figure~\ref{fig:sample_tasks}, each task contains a task 

% Take the example of differential diagnosis, where a medical professional is typically given as input a patient's medical history, symptoms, pathology and they need to produce a list of potential diagnoses with their likelihood, as well as a plan of treatment. Note that there is usually a predefined method for how diagnosis should be conducted. Performing this task then involves analyzing the input information, referring to one's own expertise and relevant domain-specific literature to form an inference, and justifying it in writing.

% \begin{itemize}
% \item \textbf{Task Objective}: A sentence about the main objective of the task.
% \item \textbf{Task Procedure}: A few sentences walking a beginner through how this task is conducted.
% \item \textbf{Input Sections}: This is the information that is typically given for the task, formatted in the form of section titles and section descriptions.
% \item \textbf{Output Sections}: This is the information that needs to be generated for the task given the input sections. This is also formatted in the form of section titles and section descriptions.
% \item \textbf{Additional Notes}: These include best practices or common mistakes, and missing context that might be important when conducting the task.
% \end{itemize}

To further set the scope for the tasks considered, we focus on tasks that meet the following criteria:
\begin{itemize}
\itemsep0em
\item \textbf{Purely textual}: Tasks can only involve writing text and should not involve other modalities in the input or output.
\item \textbf{Require domain expertise}: They can only be completed by an expert in the field.
\item \textbf{Do not require use of specific equipment or software}: They should not require operating specialized tools, equipment or software (excluding the need to search the web).
\item \textbf{Frequent}: They should be done by an expert at least once every few months.
\item \textbf{Time-consuming}: They should take a significant amount of time to complete, which can span from a half hour to a few days, but not an indefinite amount of time (for e.g., several months).
\end{itemize}

\subsection{Instantiated Examples}

Aside from task descriptions, our dataset contains examples, which are instantiations of the tasks (see Figure~\ref{fig:overview}). Concretely, we populate tasks like those shown in Figure~\ref{fig:sample_tasks} with plausible input and output sections. This process is described in \S\ref{sec:example_collection}. We require these examples to adhere to the task description such that all input and output sections from the task are present in the examples.

% Given a task, an \textbf{example} is a real sample of the input and output sections of this task with concrete details. In other words, an example is an instance of the task. In our benchmark, we consider examples that provide plausible inputs and outputs for the task. 
% Given a task description and the input sections of an example, models are then required to generate the output sections for the example.

==> sections/related.tex <==
\section{Related Work}

\paragraph{Domain-Specific NLP Benchmarks.} Using language technologies in domain-specific scenarios has the potential to help experts. Prior work has attempted to evaluate models through domain-specific benchmarks for standard tasks like question answering and summarization. The most commonly used benchmark, MMLU \citep{hendryckstest2021}, presents a collection of multiple-choice questions from various domains. Recent work has also evaluated long-form QA systems in multiple domains \citep{malaviya2024expertqa}. Beyond these, there are various benchmarks proposed in the field of law \citep{shen2022multi,niklaus-etal-2023-lextreme,guha2024legalbench}, medicine \citep{tsatsaronis2015overview,pampari-etal-2018-emrqa,jin2019pubmedqa,jin2020disease,fleming2023medalign} and other fields \citep{Rein2023GPQAAG,xia2024fofo}. A notable difference between this line of work and \textsc{Dolomites} is the task formulation (i.e., QA vs methodical tasks). As showcased in Figure~\ref{fig:quadrants}, QA involves addressing a specific information need in response to a query while conducting methodical tasks requires following a structured and consistent procedure, involving multiple steps, to complete a goal-oriented task. While this is similar in spirit to the goal of task-oriented dialog systems \citep{budzianowski-etal-2018-multiwoz}, note also that conducting our tasks require domain expertise.

\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.15]{images/dolomites_quadrants.pdf}
    \caption{Methodical tasks in \textsc{Dolomites} differ from prior NLP work as they focus on domain-specific scenarios, with a requirement to generate a long-form output.}
    \vspace{-10pt}
    \label{fig:quadrants}
\end{figure}

\paragraph{\textit{Naturalistic} Evaluation.} Evaluation that is grounded in realistic use cases, is important for reliable benchmarking of language models \cite{liao2023rethinking}. There have been a few efforts to create naturalistic benchmarks in NLP that are closely representative of real user queries. These are sometimes sourced from query logs \citep{nguyen2016ms,kwiatkowski-etal-2019-natural}, and more recently, chat histories \citep{zhao2023inthe,wildbench2024}. While these benchmarks are useful for studying model responses to generic user queries, they do not allow us to study the ability of language models to assist with domain-specific writing tasks in an isolated manner. For instance, recent work finds that user requests in chat histories often involve "planning" and "design", but these are largely ignored in model evaluations. Recent work has also advocated for evaluating models in high-risk realistic scenarios where models could operate autonomously \citep{shevlane2023model,kinniment2023evaluating}. Our work shares the motivation of setting up model evaluations that are grounded in realistic scenarios. 

\paragraph{Language Models as Writing Assistants.} Recent work has investigated the potential of language models to act as writing assistants for domain experts \citep{calderwood2020novelists,lee2022coauthor,gero2022sparks,li2024value}. While there is favorable evidence that they can improve productivity of experts \citep{noy2023experimental}, their usage has broader societal consequences, including potential impact on the workforce \citep{eloundou2023gpts}. \cite{lee2024design} present a design space that thoroughly analyzes the various considerations and implications related to their use as writing assistants. We analyze a set of societal implications that are relevant to the use of language models for our domain-specific tasks (\S\ref{sec:data}).

==> sections/results.tex <==
\section{Results and Discussion}
\label{sec:results}

\subsection{Main Results}

Our main results on the test set using all automatic metrics are reported in Table~\ref{tab:results_std}. Based on the average section presence, we note that models are largely effective at generating almost all relevant output sections from the task description. A few models (GPT-4 and Gemini-1.5-Pro) excel more at following this instruction. Based on the NLI scores, we note that the nli (reverse) scores are on average lower than nli (forward), which suggests that generated outputs contain statements not entailed by the reference. This might be because the generations contain information that is inaccurate, or they introduce new information, which may or may not be relevant. Comparing models on these scores shows that GPT-4, and Gemini-1.5-Pro produce more information that is factually consistent with the reference, while Claude-3 (both variants) and Command-R-Plus are also performant. We note that these reference-based metrics have shortcomings, as there might not just be a single reference for some of these examples, especially when the task is more subjective.

We show the win rates according to different LM evaluators in Table~\ref{tab:results_lm}. Based on these win rates, we note that a few models such as Claude-3 Opus, Gemini-1.5-Pro and Claude-3 Haiku prove to be comparable to GPT-4.

\begin{figure*}[h!]
    \centering
    \includegraphics[scale=0.3,keepaspectratio=True]{images/scores_by_field_all.pdf}
    \caption{Heatmap of scores from GPT-4, Gemini-1.5-Pro and Claude-3 Opus, aggregated by field.}
    \vspace{-5pt}
    \label{fig:scores_by_field}
\end{figure*}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\columnwidth]{images/scores_by_length.pdf}
    \caption{Heatmap of GPT-4 scores aggregated by length (in tokens) of reference output or length in terms of the number of output sections.}
    \vspace{-5pt}
    \label{fig:scores_by_length}
\end{figure}

\subsection{Results by field}

To investigate whether models perform significantly better on some fields than others, we show results by field for GPT-4, Gemini-1.5-Pro and Claude-3 Opus in Figure~\ref{fig:scores_by_field}, normalized across fields. Across all models, we find that a few fields have significantly lower NLI scores: Hospitality and Tourism, Education, and Visual Arts. Tasks from these fields sometimes involve subjectivity (for e.g., "Creating recipes with special dietary requirements", "Create a user persona for an application"), which might justify the lower NLI scores. On the other hand, tasks in fields such as Literature, History and Journalism have higher NLI scores. Some of these tasks focus more on factual reporting and narratives that may be easier to reason about.

\subsection{Results by length}

Next, we evaluate whether length of the expected output is correlated with the results of various models. Specifically, we show the results for GPT-4 split into bins by the 1) length of the reference outputs and 2) the number of output sections expected for the task. These results are normalized across bins and shown in Figure~\ref{fig:scores_by_length}. We find that examples which require longer outputs are significantly harder for models. This is supported by the fact that examples with longer expected outputs (both in terms of tokens and number of outputs sections) have significantly lower NLI scores.

\subsection{Error Analysis}

We analyze generated outputs from the top-3 models for examples where the end-to-end NLI scores are lowest. Broadly, we find the failure cases of models to belong to the following categories:

\begin{itemize}
    \item Lacking depth: Writing technical or scientific documents requires depth and focus, which was sometimes found to be lacking. For instance, in a task on writing up a report on an experimental study in clinical psychology, the output was lacking concrete statistical results and method details. Similarly, models sometimes diverged to enumerating many potentially relevant topics.
    \item Verbose outputs: A common characteristic of some model outputs was their verbosity. Common patterns included defining jargons when not necessary, and generating many filler statements that don't add much content.
    \item Missing information: There were a few cases where an output section required producing multiple pieces of information (for eg, a budget breakdown and project timeline), but the model entirely missed producing one.
    \item Subjectivity: We came across tasks from various fields that are subjective or require creativity (for eg, \textit{Creating recipes with special dietary requirements}). Traditional reference-based measures such as NLI are not capable of handling this subjectivity during evaluation. Future work will explore how we can evaluate subjective outputs with no single reference.
    \item 
\end{itemize}

==> tables/edit_stats.tex <==
% \setlength{\tabcolsep}{10pt} % Default value: 6pt

% \renewcommand{\arraystretch}{1.5} % Default value: 1

% \begin{table*}[h!]
% \centering
% \scalebox{.8}{
% \begin{tabular}{ lccccc }
% \rowcolor{gray!40}
%  & \textbf{Avg Length} & \textbf{\makecell{Avg section\\presence \%($\uparrow$)}} & \textbf{\makecell{Flesch-Kincaid\\Grade Level ($\uparrow$)}} &  \textbf{\makecell{Gunning-Fog\\Index ($\uparrow$)}} & \textbf{SMOG Index ($\uparrow$)} \\ \toprule
% \texttt{original} & 388.98 & 92.81 & 11.69 & 15.25 & 13.06 \\
% \texttt{post-edited} & 590.24 & 97.67 & 13.46 & 17.24 & 14.35 \\
%  \bottomrule
% \end{tabular}
% }
% \caption{Statistics of the original and post-edited examples in \textsc{Dolomites}.}
% \label{tab:edit_stats}
% \end{table*}

% \setlength{\tabcolsep}{10pt} % Default value: 6pt

\renewcommand{\arraystretch}{1.4} % Default value: 1

\begin{table}[t!]
\centering
\scalebox{.7}{
\begin{tabular}{ lccccc }
\rowcolor{gray!40}
 & \textbf{Avg Length} & \textbf{\makecell{Avg section\\presence \%($\uparrow$)}} & \textbf{\makecell{Flesch-Kincaid\\Grade Level ($\uparrow$)}} \\ \toprule
\texttt{original} & 388.98 & 92.81 & 11.69 \\
\texttt{post-edited} & 590.24 & 97.67 & 13.46  \\
 \bottomrule
\end{tabular}
}
\caption{Statistics of the original and post-edited examples in \textsc{Dolomites}.}
\label{tab:edit_stats}
\vspace{-10pt}
\end{table}

==> tables/main_paper_example.tex <==
\begin{table*}[t!]
    \centering
    \rowcolors{2}{blue!10}{blue!10}
    \begin{tabular}{|p{\dimexpr0.5\linewidth-2\tabcolsep-\arrayrulewidth\relax}|p{\dimexpr0.5\linewidth-2\tabcolsep-\arrayrulewidth\relax}|}
        \toprule
        \multicolumn{2}{|p{2\columnwidth}|}{\cellcolor{blue!25}\textbf{Sample Task and Example from \textsc{Dolomites}}} \\
        \midrule
        \multicolumn{2}{|p{2\columnwidth}|}{\cellcolor{blue!10}\raggedright \tiny \texttt{\textbf{\underline{TASK DESCRIPTION}} \linebreak \linebreak \textbf{Task Objective}: Writing a funding application for a medical research project. \linebreak \linebreak \textbf{Task Procedure}: To write a funding application for a research project, you need to start with a clear and concise idea for the research project, identify matching funding sources, understand the funder's priorities. Then, write a detailed project description and prepare a specific budget. Complete the application form provided by the funder and follow all guidelines. Review the application, submit it, and await feedback. \linebreak \linebreak \textbf{Additional Notes}: It is important to clearly define the research idea, understand the funder's priorities, write a detailed project description, prepare a specific budget, and review before submitting. Common mistakes include overlooking eligibility, using jargon, poor structure of the application, and an overwhelming page layout. \linebreak \linebreak \textbf{Input Sections}: \linebreak \linebreak * \textbf{Project Idea}: 1 paragraph. A clear and concise idea for the research project is essential. \linebreak \linebreak * \textbf{Potential Funding Sources}: 1 paragraph. Estimated cost and identification of potential funding sources that align with the research topic. \linebreak \linebreak \textbf{Output Sections}: \linebreak \linebreak * \textbf{Funding application}: 2 paragraphs. The funding application will include a summary, an introductory section including background and motivation, detailed project description, and detailed budget. \linebreak \linebreak * \textbf{Timeline}: In addition, a detailed timeline with key milestones is essential to demonstrate preparedness and careful planning for the project.}} \\ \midrule
        \multicolumn{2}{|p{2\columnwidth}|}{\cellcolor{blue!10}\raggedright \tiny \texttt{\textbf{\underline{EXAMPLE INPUT}} \linebreak \linebreak * \textbf{Project Idea}: Our research aims to develop a novel digital intervention that combines multi-faceted online self-management support with remote patient monitoring to improve disease understanding, treatment adherence, and clinical outcomes for patients recently hospitalized with an acute exacerbation of COPD. This intervention will leverage the capabilities of the  myCOPD app, which provides a comprehensive platform for education, pulmonary rehabilitation, inhaler technique videos, and environmental alerts. By integrating remote monitoring through clinician interfaces, we aim to facilitate timely intervention and personalized care for this vulnerable patient population. \linebreak \linebreak * \textbf{Potential Funding Sources}: The estimated cost of this research project is \$500,000. We have identified the  following potential funding sources that align with our research topic: \linebreak * National Heart, Lung, and Blood Institute (NHLBI) \linebreak * National Institute of Health (NIH) \linebreak * American Lung Association}} \\ \midrule
        \multicolumn{2}{|p{2\columnwidth}|}{\cellcolor{blue!10}\raggedright \tiny \texttt{\textbf{\underline{EXAMPLE OUTPUT}}  \linebreak \linebreak * \textbf{Funding Application}: \linebreak \linebreak \textbf{Summary}: This research project proposes the development and evaluation of a novel digital intervention to improve clinical outcomes for COPD patients recently discharged from   the hospital. The intervention combines the myCOPD app with remote patient monitoring to enhance disease understanding, treatment adherence, and timely intervention. \linebreak \linebreak \textbf{Background and Motivation}: COPD is a significant public health concern, and acute exacerbations often lead to hospitalizations. Post-discharge management is crucial, but patients face challenges with self-management and access to care. Digital interventions have shown promise in improving COPD outcomes, and remote monitoring enables proactive care. Our proposed intervention aims to address these challenges by providing comprehensive support and personalized monitoring for vulnerable COPD patients. \linebreak \linebreak \textbf{Project Description}: We will conduct a randomized controlled trial to evaluate the efficacy of our digital intervention. Patients recently hospitalized with COPD  will be randomized to either the intervention group or standard of care. The intervention group will receive access to the myCOPD app and remote monitoring by their healthcare team. The app will enable the patient to self-report their symptoms and will provide a personalized COPD action and management plan, educational materials, a gated pulmonary rehabilitation program, inhaler technique videos, environmental alerts, and prescription assessment to cross-check prescribed medicine and identify any conflicts. The app will be coupled with smart inhalers and indoor air quality sensors that collect data from the patient indoor environment. Data collection through the myCOPD app will include self-reported symptoms, adherence to treatment, and indoor air quality. The clinician interface will allow for real-time monitoring of patient symptoms, adherence to treatment plan, and environmental triggers. The standard of care group will receive written self-management advice. We will assess clinical outcomes, including exacerbation rates, hospital readmissions, and quality of life. Assessment of outcomes will be performed by a dedicated team of healthcare professionals and data analysts. This will be done by leveraging the comprehensive data collected through the myCOPD app and from linked electronic health care records. \linebreak \linebreak \textbf{Budget}: The total budget for this project is \$500,000, which includes personnel costs, equipment, supplies, and travel expenses. The budget includes: \linebreak * Personnel Costs: \$350,000. This includes salaries for all researchers, technicians, and research administrators involved in the project. \linebreak * Data Collection and Analysis: \$70,000. This covers the costs  associated with gathering the necessary data for our research and the subsequent analysis. \linebreak * Supplies: \$30,000. This allocation is for the procurement of all necessary supplies and materials required for the project such as laboratory test kits, hardware, and software licences. \linebreak * Travel and Publication Expenses: \$50,000, which include the cost of staff and patient travel, conference attendance, and publication of finding in top-tier academic journals. \linebreak \linebreak * \textbf{Timeline}: \linebreak * Year 1: Development and pilot testing of the digital intervention \linebreak * Year 2: Recruitment and enrollment of participants \linebreak * Year 3: Data collection and analysis \linebreak * Year 4: Dissemination of results \linebreak \linebreak We believe that this research has the potential to significantly improve the care and outcomes for COPD patients. By leveraging technology and providing personalized support, we aim to empower patients to better manage their condition and reduce the burden of this chronic disease.}} \tabularnewline
        \bottomrule
    \end{tabular}
    \caption{We show here an example of a task description from \textsc{Dolomites} as well as an example of this task.}
    \label{tab:sample_example}
\end{table*}


==> tables/results_autoraters.tex <==
\begin{table}[!ht]
\centering
\scalebox{.65}{
\begin{tabular}{lccc}
\rowcolor{gray!40}
    \toprule
    \textbf{Model} & \textbf{\makecell{Win rate\\(GPT-4)}} & \textbf{\makecell{Win rate\\(Claude-3 Opus)}} & \textbf{\makecell{Win rate\\(Gemini-Ultra)}} \\
    \midrule
    \texttt{Claude-3 Haiku} & 43.0 & 50.0 & \\
    \texttt{Claude-3 Opus} & 50.0 & 54.5 & \\
    \texttt{Command-R-Plus} & 32.0 & 44.0 & \\
    \texttt{Gemini-1.5-Pro} & 48.0 & 49.0 & \\
    \texttt{Gemini-MPP} & 52.0 & 61.5 & \\
    \texttt{Gemini-Pro} & 17.0 & 21.0 & \\
    \texttt{GPT-3.5-Turbo} & 15.0 & 16.0 & \\
    \texttt{GPT-4} & 50.0 & 50.0 & \\
    \texttt{Mistral-Large} & 29.0 & 27.5 & \\
    \texttt{Mixtral-8x7B} & 20.0 & 24.0 & \\
    \texttt{OLMo-7B-Instruct} & 4.0 & 8.0 & \\
    \bottomrule
\end{tabular}
}
\caption{Results on the \textsc{Dolomites} benchmark using various LM-based judgements.}
\label{tab:results_lm}
\end{table}

==> tables/results_std_and_nli.tex <==
\begin{table*}[!t]
\centering
\scalebox{.7}{
\setlength\tabcolsep{3pt} % Adjust the horizontal padding here
\begin{tabular}{@{}l@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{}}
\rowcolor{gray!40}
    \toprule
    \textbf{Model} & \textbf{\makecell{Avg\\Length}} & \textbf{\makecell{Avg Section\\Presence \%}} & \textbf{BLEU-1} & \textbf{BLEU-4} & \textbf{BLEURT} & \textbf{ROUGE-L} & \textbf{\makecell{F1\\Overlap}} & \textbf{\makecell{nli \\ (forward)}} & \textbf{\makecell{nli \\ (reverse)}} & \textbf{\makecell{nli \\ (h-mean)}} \\
    \midrule
    \texttt{Claude-3 Haiku} & 378.64 & 92.42 & \textbf{0.3909} & 0.1077 & 0.4232 & \textbf{0.2416} & \textbf{0.4619} & 0.4218 & 0.3664 & 0.3922 \\
    \texttt{Claude-3 Opus} & 411.17 & 92.25 & 0.3859 & \textbf{0.1090} & 0.4180 & 0.2414 & 0.4596 & 0.3739 & 0.3851 & 0.3794 \\
    \texttt{Command-R-Plus} & 435.98 & 93.39 & 0.3658 & 0.0827 & 0.4094 & 0.2141 & 0.4350 & 0.4004 & 0.3664 & 0.3826\\
    \texttt{Gemini-1.5-Pro} & 344.19 & 95.91 & 0.3920 & 0.1046 & 0.4164 & 0.2383 & 0.4614 & \textbf{0.4255} & 0.3947 & 0.4095\\
    \texttt{Gemini-Pro} & 267.26 & 93.92 & 0.3557 & 0.0954 & 0.4157 & 0.2270 & 0.4413 & 0.3451 & 0.3082 & 0.3256 \\
    \texttt{GPT-3.5-Turbo} & 240.30 & 89.79 & 0.3335 & 0.0958 & \textbf{0.4296} & 0.2317 & 0.4400 & 0.3981 & 0.3020 & 0.3434 \\
    \texttt{GPT-4} & 401.97 & \textbf{96.07} & 0.3810 & 0.0941 & 0.4184 & 0.2285 & 0.4505 & 0.4098 & \textbf{0.4121} & \textbf{0.4109} \\
    \texttt{Mistral-Large} & 320.95	& 92.69 & 0.3917 & 0.1098 & 0.4180 & 0.2410 & 0.4619 & 0.3675 & 0.3596 & 0.3635 \\
    \texttt{Mixtral-8x7B} & 379.80 & 87.28 & 0.3634 & 0.1002 & 0.4136 & 0.2290 & 0.4345 & 0.3399 & 0.3087 & 0.3236 \\
    \texttt{OLMo-7B-Instruct} & 776.95 & 73.83 & 0.2580 & 0.0618 & 0.3953 & 0.1782 & 0.3262 & 0.2072 & 0.1817 & 0.1936 \\
    \bottomrule
\end{tabular}
}
\caption{Results on the \textsc{Dolomites} benchmark with conventional generation metrics as well as factual consistency using NLI models.}
\label{tab:results_std}
\end{table*}

==> tables/results_std_and_nli_test_mirella.tex <==
\begin{table}[t]
\centering
\scalebox{.75}{
  %\setlength\tabcolsep{1pt} % Adjust the horizontal padding here
  \setlength\extrarowheight{-4pt}
\begin{tabular}{l@{~}c@{~~}c@{~~}c@{~~}c@{~~}c@{~~}c@{~~}c}
    \toprule
    \rowcolor{gray!40}
    \textbf{Model} & \textbf{\makecell{AvgL}} & \textbf{\makecell{AvgS}} & \textbf{BRT} & \textbf{RL} & \textbf{\makecell{Fnli}} & \textbf{\makecell{Rnli}} & \textbf{\makecell{Mnli}} \\
    \midrule
    \texttt{Claude-3 Haiku} & 376.49 & 91.97  & 0.42 & 0.24 & 0.40 &  0.30 & 0.38 \\
    \texttt{Claude-3 Opus} & 417.41 & 91.53   & 0.42 & \textbf{0.24} & 0.36  & 0.30 & 0.37 \\
    \texttt{Command-R-Plus} & 440.44 & 92.92  & 0.41 & 0.21 & 0.39 &  0.30 & 0.38 \\
    \texttt{Gemini-1.5-Pro} & \textbf{349.27} & 95.25  & 0.41 & \textbf{0.24} & \textbf{0.41} &0.38 & 0.39 \\
    \texttt{Gemini-MPP} & \textbf{361.87} & \textbf{95.74}      & 0.41 & \textbf{0.24} & \textbf{0.40} &  \textbf{0.40} & \textbf{0.40} \\
    \texttt{Gemini-Pro} & 269.68 & 93.61      & 0.41 & 0.23 & 0.34 &  0.31 & 0.32 \\
    \texttt{GPT-3.5-Turbo} & 240.89 & 88.98   & \textbf{0.43} & 0.23 & 0.39 &  0.29 & 0.33 \\
    \texttt{GPT-4} & 407.35 & \textbf{95.46}           & 0.42 & 0.23 & 0.39 &  \textbf{0.40} & \textbf{0.40} \\
    \texttt{Mistral-Large} & 327.12 & 92.61   & 0.42 & \textbf{0.24} & 0.35 &  0.35 & 0.35 \\
    \texttt{Mixtral-8x22B} & 386.61 & 88.39    & 0.41 & 0.23 & 0.33 &  0.31 & 0.32 \\
    \texttt{Mixtral-8x7B} & 386.61 & 88.39    & 0.41 & 0.23 & 0.33 &  0.31 & 0.32 \\
    \texttt{OLMo-7B-Instruct} & 784.22 & 74.02&  0.39 & 0.18 &  0.19) &  0.17 & 0.18 \\
    \bottomrule
\end{tabular}
}
\caption{Results on the \textsc{Dolomites} test set using automatic
  evaluation metrics.  AvgL/S  denotes the average output
  length/section presence, RL is a shorthand for ROUGE-L, and
  F/R/Mnli refer to forward, reverse and (harmonic) mean NLI.}
\label{tab:results_std}
\end{table}



==> tables/tasks.tex <==
\setlength{\tabcolsep}{6pt} % Default value: 6pt

\renewcommand{\arraystretch}{1.15} % Default value: 1
\definecolor{Lavender}{rgb}{0.9,0.9,0.98}

\begin{table*}[t!]
\centering
% \footnotesize
\scalebox{.75}{
\rowcolors{2}{Lavender!55}{white}
\begin{tabular}{ c c p{12cm} }
\rowcolor{Lavender!80}
\textbf{Field} & \textbf{Number of Tasks} & \textbf{Sample Task Objective} \\ \toprule
 Anthropology & 8 & \textit{Design a survey focused on examining specific cultural practices, rituals, and societal norms within a chosen cultural group or community} \\
 Architecture & 20 & \textit{Developing a construction phasing plan for a building project}  \\
 Biology & 21 & \textit{Developing a protocol for a toxicity assay}  \\
 Business & 26 & \textit{Writing a section of a non-financial report for a client, focusing on a company's environmental and social activities}  \\
 Chemistry & 21 & \textit{To write a retrosynthesis scheme/plan for a specific target molecule} \\
 Economics & 17 & \textit{Reviewing investment options for advising companies} \\
 Education & 23 & \textit{To create a lesson plan for a school class} \\
 Engineering \& Technology & 22 & \textit{To write the instructions for conducting a radioactive experiment.} \\
 Environmental Science & 23 & \textit{Writing the life cycle assessment of a system, product or process} \\
 Geography & 20 & \textit{Analyzing the environmental and social impacts of illegal mining activities in a specific region} \\
 History & 22 & \textit{Summarize and analyze a specific medieval legal code} \\
 Hospitality \& Tourism & 21 & \textit{Adapt existing recipes to cater to various dietary preferences} \\
 Journalism & 20 & \textit{Write a news story based on an interview} \\
 Law & 38 & \textit{Drafting a petition to challenge a decision} \\
 Linguistics & 20 & \textit{Carry out a short literature review of a given problem in linguistics} \\
 Literature & 20 & \textit{To write a research proposal for a presentation at a literary research conference} \\
 Mathematics & 15 & \textit{Writing an experimental setup suitable for testing a research hypothesis in applied mathematics} \\
 Medicine & 24 & \textit{Writing a list of potential radiotherapy regimens for a cancer patient} \\
 Music & 23 & \textit{Writing lyrics for a game's soundtrack} \\
 Philosophy & 13 &  \textit{Provide ethical recommendations for patient/doctor cases} \\
 Physics \& Astronomy & 21 & \textit{Design specifications for a pump or turbine system}  \\
 Political Science & 20 & \textit{Redline a management measure / legislative policy}  \\
 Psychology & 21 & \textit{Writing a study protocol of a neuroimaging research project} \\
 Sociology & 20 & \textit{Analyzing responses from sociological interviews to identify themes relevant to the research question} \\
 Visual Arts & 20 & \textit{The objective of this task is to write a catalog entry for an art exhibition} \\
 \bottomrule
\end{tabular}
}
\caption{Fields represented in \textsc{Dolomites}, with the number of tasks and a sample task from each field.}
\label{tab:tasks_all}
\end{table*}
